FocusFormer: Focusing on What We Need via Architecture Sampler

Vision Transformers (ViTs) have underpinned the recent breakthroughs in computer vision. However, designing the architectures of ViTs is laborious and heavily relies on expert knowledge. To automate the design process and incorporate deployment flexibility, one-shot neural architecture search decouples the supernet training and architecture specialization for diverse deployment scenarios. To cope with an enormous number of sub-networks in the supernet, existing methods treat all architectures equally important and randomly sample some of them in each update step during training. During architecture search, these methods focus on finding architectures on the Pareto frontier of performance and resource consumption, which forms a gap between training and deployment. In this paper, we devise a simple yet effective method, called FocusFormer, to bridge such a gap. To this end, we propose to learn an architecture sampler to assign higher sampling probabilities to those architectures on the Pareto frontier under different resource constraints during supernet training, making them sufficiently optimized and hence improving their performance. During specialization, we can directly use the well-trained architecture sampler to obtain accurate architectures satisfying the given resource constraint, which significantly improves the search efficiency. Extensive experiments on CIFAR-100 and ImageNet show that our FocusFormer is able to improve the performance of the searched architectures while significantly reducing the search cost. For example, on ImageNet, our FocusFormer-Ti with 1.4G FLOPs outperforms AutoFormer-Ti by 0.5% in terms of the Top-1 accuracy.

==> preliminary.tex <==
\subsection{Vision transformer}


\subsection{Neural architecture search}
Neural architecture search (NAS)~\cite{zoph2016neural,pham2018efficient,liu2018darts} seeks to find architectures with promising performance while satisfying the resource constraint $B$, which can be formulated as
\begin{equation}
\begin{aligned}
    \label{eq:nas_problem}
    \min_{\alpha}&\mL_{\mathrm{val}}(W_{\alpha}^*; \mD_{\mathrm{val}}) \\
    \st~ W_{\alpha}^* = \arg\min_{W_{\alpha}}&\mL_{\mathrm{train}}(W_{\alpha}; \mD_{\mathrm{train}}),~C(\alpha) < B,
\end{aligned}  
\end{equation}
where $W_{\alpha}$ is the weights of network architecture $\alpha$, $C(\alpha)$ is the computational cost of $\alpha$, and $\mL_{\mathrm{train}}$ and $\mL_{\mathrm{val}}$ are the training loss and validation loss, respectively. Here, $\mD_{\mathrm{train}}$ and $\mD_{\mathrm{val}}$ are the training and validation dataset, respectively. To solve Problem~(\ref{eq:nas_problem}), for each architecture $\alpha$, we has to train weights $W_{\alpha}$
until convergence to obtain $W_{\alpha}^*$, which takes unbearable computational cost.


To solve this issue, one-shot NAS~\cite{Cai2020Once-for-All,guo2020single,Fan2020Reducing,xu2021autoformer,chen2021searching} has been proposed to decouple the model training stage and architecture search stage. In the model training stage, the goal is to train an over-parameterized supernet that supports many sub-networks of different configurations with the shared parameters to accommodate different deployment scenarios. Let $W$ be the weights of the supernet. The objective function for the supernet training can be formulated as
\begin{equation}
    \label{eq:objective_one_shot}
     W^* = \arg\min_W \mathbb{E}_{\alpha \in \mA}\left[ \mL_{\mathrm{train}}(S(W, \alpha)) \right],
\end{equation}
where $S(W, \alpha)$ is a selection function that chooses a part of parameters from $W$ to constitute the sub-network with architecture configuration $\alpha$ and $\mA$ is the architecture search space. To solve Problem~(\ref{eq:objective_one_shot}), existing methods~\cite{guo2020single,Cai2020Once-for-All} assume that all the sub-networks are equally important and use a uniform sampling strategy to approximate the expectation term. For the architecture search stage, we obtain the specialized sub-network that satisfies the resource constraint $B$ given a deployment scenario while maximizing the validation accuracy $\mathrm{Acc}_{\mathrm{val}}(S(W^*, \alpha))$, which can be formulated as
\begin{equation}
    \begin{aligned}
    \label{eq:search_objective}
    \max_{\alpha}&~\mathrm{Acc}_{\mathrm{val}}(S(W^*, \alpha)) \\
    \st&~ C(\alpha) < B.
    \end{aligned}
\end{equation}
Here, $W^*$ is the well-learned weight of the supernet in the model training stage. Except for the validation accuracy, we can also use the negative validation loss to measure the performance of the searched architectures. Since the supernet has been well-trained, we are able to obtain any sub-network without any fine-tuning or retraining during architecture search, which yields a much lower search cost compared with Problem~(\ref{eq:nas_problem}).

